Memory-Efficient Object-Oriented Programming on GPUs

Object-oriented programming is often regarded as too inefficient for high-performance computing (HPC), despite the fact that many important HPC problems have an inherent object structure. Our goal is to bring efficient, object-oriented programming to massively parallel SIMD architectures, especially GPUs. In this thesis, we develop various techniques for optimizing object-oriented GPU code. Most notably, we identify the object-oriented Single-Method Multiple-Objects (SMMO) programming model. We first develop an embedded C++ Structure of Arrays (SOA) data layout DSL for SMMO applications. We then design a lock-free, dynamic memory allocator that stores allocations in SOA layout. Finally, we show how to further optimize the memory access of SMMO applications with memory defragmentation.

==> Makefile <==
APP := main

LATEX := pdflatex
BIBTEX := bibtex
LATEX_FLAGS := -shell-escape -halt-on-error -synctex=1

.PHONY: all clean distclean

.SUFFIX: .tex .pdf

%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(BIBTEX) $(APP)
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<

all: $(APP).pdf

distclean:
	$(RM) $(APP).pdf

clean:
	$(RM) *~ $(APP).dvi $(APP).aux $(APP).toc $(APP).out \
	$(APP).log $(APP).pdf $(APP).ps $(APP).blg

